A parabolic local problem with exponential decay of the resonance error for numerical homogenization

This paper aims at an accurate and efficient computation of effective quantities, e.g., the homogenized coefficients for approximating the solutions to partial differential equations with oscillatory coefficients. Typical multiscale methods are based on a micro-macro coupling, where the macro model describes the coarse scale behaviour, and the micro model is solved only locally to upscale the effective quantities, which are missing in the macro model. The fact that the micro problems are solved over small domains within the entire macroscopic domain, implies imposing artificial boundary conditions on the boundary of the microscopic domains. A naive treatment of these artificial boundary conditions leads to a first order error in $\varepsilon/\delta$, where $\varepsilon < \delta$ represents the characteristic length of the small scale oscillations and $\delta^d$ is the size of micro domain. This error dominates all other errors originating from the discretization of the macro and the micro problems, and its reduction is a main issue in today's engineering multiscale computations. The objective of the present work is to analyze a parabolic approach, first announced in [A. Abdulle, D. Arjmand, E. Paganoni, C. R. Acad. Sci. Paris, Ser. I, 2019], for computing the homogenized coefficients with arbitrarily high convergence rates in $\varepsilon/\delta$. The analysis covers the setting of periodic micro structure, and numerical simulations are provided to verify the theoretical findings for more general settings, e.g. random stationary micro structures.

==> tex/ALTER_2D_num_exp_2.tex <==
We consider the upscaling of the $2\times 2$ isotropic tensor:
\begin{equation}\label{eq: tensor GloriaLeBris}
a(\bx) = \left( \frac{2 + 1.8 \sin(2\pi x_1)}{2 + 1.8 \cos(2\pi x_2)} + \frac{2 + \sin(2\pi x_2)}{2 + 1.8 \cos(2\pi x_1)} \right)\textrm{Id}  
\end{equation}
for which the homogenized tensor is
\begin{equation*}
a^0 \approx
\begin{pmatrix}
2.757 & -0.002\\
-0.002 & 3.425
\end{pmatrix} .
\end{equation*}
%while the correction part is 
%\begin{equation*}
%a_{corr}^0 \approx 
%\begin{pmatrix}
%-1.832 & -0.002\\
%-0.002 & -1.164
%\end{pmatrix}.
%\end{equation*}
Here, we compare the performances of the described parabolic approach (``par.'' in the legends), the standard elliptic approach (``ell.'' in the legends) \add{and the regularized elliptic approach of Ref. \refcite{Glo11}}. 
In comparing the \del{two} \add{different} methods, we used a filtered version of \eqref{eq:bar_a0_Intro}, namely
 \begin{equation}
 \mathbf{e}_i \cdot a^{0}_{R,L} \mathbf{e}_j := \int_{K_L} \mathbf{e}_i \cdot a(\bx) \left( \mathbf{e}_j + \nabla \chi_R^j(\bx) \right) \mu_L(\bx)\,d\bx, 
 \end{equation}
%
\corr{that improves the error constant for the classical approach. However, we recall that} the standard elliptic method provides a first order convergence rate, independently of the use of oversampling or filtering, as shown in Ref. \refcite{YuE07}. 
By contrast, the use of high order filters in the parabolic \add{and regularized elliptic} schemes improves the convergence rate without affecting the computational cost. 
\del{The two }\add{All the} approaches are solved using $\mathbb{P}1$ finite element discretization in space with $64$ points per periodic cell. Mass lumping has been used in order to perform the time integration, which is carried out via the ROCK4 method, see Ref. \refcite{Abd02}, with $tol=10^{-6}$. Finally Simpson's quadrature rule is used for computing the time integral defining homogenized coefficients. 

Results are depicted in \cref{fig:compare}. As expected, one cannot reach a convergence rate higher than 1 for the standard elliptic approach, in contrast to the parabolic method. We notice a longer ``flat'' region in the convergence plot for small values of $k_o$ and high order filters. Intuitively, for any given $R$, the region where the filter is ``not almost zero'' decreases for smaller $k_o$ and larger $q$. Hence, we need larger values of $R$ for the averaging integral to contain enough data and the error to decrease with the expected rate.
%
%\begin{figure}[h!]
%\begin{subfigure}{.45\textwidth}
%	\centering
%	\input{"../img/GloriaLeBris/compare q=4 L = 0.50R errorTot"}
%	\caption{ }
%\end{subfigure}
%\begin{subfigure}{.45\textwidth}
%	\centering
%	\input{"../img/GloriaLeBris/compare L = 0.33R errorTot"}
%	\caption{}
%\end{subfigure}
%\caption{}
%\label{fig:boh3}
%\end{figure}
%
%\begin{figure}[t]
%	\centering
%	\input{"../img/GloriaLeBris/compare q=4 L = 0.50R errorTot"}
%	\caption{Comparison of the modelling error for tensor \cref{eq: tensor GloriaLeBris}. Filter's order $q=4$ and $L=R/2$.}
%	\label{fig:compare q=4 L = 0.50R}
%\end{figure}
%
%\begin{figure}[t]
%	\centering
%	\input{"../img/GloriaLeBris/compare L = 0.33R errorTot"}
%	\caption{Comparison of the modelling error for tensor \cref{eq: tensor GloriaLeBris}. Filter's order $q$ and $L=R/3$.}
%	\label{fig:compare L = 0.33R}
%\end{figure}
%
%\begin{figure}[h!]
%	\centering
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/GloriaLeBris/compare standard q=2 L = 0.33R errorTot"}
%	\end{subfigure}
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/GloriaLeBris/compare standard q=2 L = 0.50R errorTot"}
%	\end{subfigure}	
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/GloriaLeBris/compare standard q=4 L = 0.33R errorTot"}
%	\end{subfigure}
%	\begin{subfigure}{.45\textwidth}
%		\input{"../img/GloriaLeBris/compare standard q=4 L = 0.50R errorTot"}
%	\end{subfigure}	
%	\caption{Comparison of the modelling error for tensor \cref{eq: tensor GloriaLeBris}.}
%	\label{fig:compare2}
%\end{figure}
%
\begin{figure}
	\centering
	\begin{subfigure}{.45\textwidth}
		\input{"../img/GloriaLeBris/compare Gloria q=1 L = 0.33R errorTot"}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\input{"../img/GloriaLeBris/compare Gloria q=1 L = 0.67R errorTot"}
	\end{subfigure}	
	%
	\begin{subfigure}{.45\textwidth}
		\input{"../img/GloriaLeBris/compare Gloria q=3 L = 0.33R errorTot"}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\input{"../img/GloriaLeBris/compare Gloria q=3 L = 0.67R errorTot"}
	\end{subfigure}	
	%
	\begin{subfigure}{.45\textwidth}
		\input{"../img/GloriaLeBris/compare Gloria q=5 L = 0.33R errorTot"}
	\end{subfigure}
	\begin{subfigure}{.45\textwidth}
		\input{"../img/GloriaLeBris/compare Gloria q=5 L = 0.67R errorTot"}
	\end{subfigure}	
	\caption{Comparison of the resonance error in the elliptic and parabolic models for tensor \cref{eq: tensor GloriaLeBris}.}
	\label{fig:compare}
\end{figure}

==> tex/ALTER_numerical_results3.tex <==
In this section we present several numerical tests which support the theoretical results of \Cref{sec:analysis} and experimentally verify the resonance error bound of \cref{thm: modelling error parabolic correctors filter}. 
We \corr{illustrate} the expected convergence rates by varying the regularity parameter $q$ of the filters, in a periodic, smooth setting, as rigorously proven in the previous sections. Additionally, we compare the convergence rate of the resonance error for the parabolic scheme with that of standard numerical homogenization scheme. We also test non-smooth periodic and stochastic coefficients, which violate the theoretical assumptions in the analysis. \corr{Nevertheless, we obtain} results as in the smooth periodic case.

In order to numerically assess the convergence rate of the resonance error, we compute the approximations of the homogenized tensor through the described parabolic cell problems on domains of increasing size, $R\in[1,20]$, and calculate the Frobenius norm of the difference between such approximations and the exact $a^0$. 
In the case of periodic coefficients whose homogenized value could not be known exactly (i.e., without discretization error) the reference value is computed by solving the standard elliptic micro problem \cref{eq:periodic micro} with $R=1$ and periodic boundary conditions and using formula \cref{eq:a0}. 
In the random setting no approximation is available without some resonance error. 
In this case, we \corr{take as reference value for the homogenized tensor the one computed from the numerical approximation of the parabolic correctors over the largest domain $R_{max}=20$.}

To compute a numerical approximation of $a^{0}_{R,L,T}$, we use a Finite Elements (FE) discretization for the micro problems \cref{eq:parabolic dirichlet problem} in space, and a stabilised explicit Runge-Kutta method with adaptive time stepping for the time discretization. A high (fourth) order method, Ref. \refcite{Abd02}, is chosen in order to make the temporal discretization error negligible with respect to the resonance error. As we use explicit methods in time, we need a mass matrix that is cheap to invert. This is achieve by using either mass lumping (for low order FEMs) or discontinuous Galerkin methods (for arbitrary order FEMs).

%Whichever method one chooses, it is advisable to use an adaptive time stepping scheme in order to exploit the smoothing properties of the parabolic equations. 
As a second step, the upscaled tensor is approximated by a double integration in space and time. \corr{The spatial integral of the parabolic correctors is computed by using} the FE filtered mass matrix of components
\begin{equation*}
m_{ij} = \int_{K_L} \phi_i(\bx) \phi_j(\bx) \mu_L(\bx) \,d\bx,
\end{equation*}
where $\{\phi_i\}_i$ are the FE basis functions.
The integration in time is performed by the use of Newton-Cotes formulae for non-uniform discretizations.

In order to optimize the convergence rate of the error with respect to the sampling domain size $R$, we take the optimal values of \cref{thm: modelling error parabolic correctors filter} for the averaging domain size $L$ ($K_L\subset K_R$) and for the final time $T$ given by 
$$L = k_o R, \text{ and } T = \frac{R-L}{\sqrt{8\beta \lambda_0}},$$	 
where $\beta$ is the continuity constant of the tensor $a$ and $\lambda_0$ is the smallest eigenvalue of the elliptic operator $-\nabla\cdot\left(a(\cdot)\nabla\right)$ with periodic boundary conditions. The oversampling ratio, $0<k_o<1$, and the order of filters, $q$, can be chosen freely.

==> tex/ALTER_proofGreenFunction.tex <==
In this section we provide an alternative proof to \cref{lemma: preliminary estimate sup-theta}. As a first step, we provide an upper bound estimate on the gradient of the parabolic Green's function, which will be utilized subsequently. The proof of such an estimate is based on the well-known Nash-Aronson estimates and the parabolic Caccioppoli inequality.
The Nash-Aronson estimate, Ref. \refcite{Aro67,Aro68}, bounds the infinite domain Green's function $\Gamma_{\infty}(x,t;y,s)$ in a pointwise sense. Such an estimate remains true for the Green's function on bounded domains with Dirichlet boundary conditions. Indeed, denoted $\Gamma_{\Delta}:=\Gamma_{\infty}-\Gamma$ and from the continuity of the functions, the maximum principle implies $\Gamma_{\Delta}\ge 0$. Thus, 
\begin{equation*}
	\Gamma(x,t;y,s)\le\Gamma_{\infty}(x,t;y,s)\le \frac{C}{t^{d/2}} e^{-c\frac{\abs{x-y}^2}{t}}.
\end{equation*}
The parabolic Caccioppoli inequality is stated in the \Cref{lemma: caccioppoli} and it is proved, e.g., in \S 1, Chapter 8, Ref. \refcite{AKM19}. 
For sake of readability, we define
\begin{equation*}
	Q_r(\bx,t):= (t-r^2,t)\times B_r(\bx).
\end{equation*}
\begin{lemma}\label{lemma: caccioppoli}
	Let $u\in L^2\left((t-4r^2,t),H^1\left(B_{2r}(\bx)\right)\right)$ solve
	\begin{equation*}
		\partial_t u - \nabla\cdot\left(a(\bx)\nabla u \right)=0, \quad \text{in }Q_r(\bx,t).
	\end{equation*}
	There exists a constant $C(d,\alpha,\beta)\le \infty$ such that
	\begin{equation*}%\label{eq:caccioppoli inequality}
		\norm{\nabla u}_{L^2\left(Q_r(\bx,t)\right)}
		\le
		\frac{C}{r} \norm{u}_{L^2\left(Q_{2r}(\bx,t)\right)}.
	\end{equation*}
\end{lemma}
\begin{lemma}\label{lemma:bound gradient green}
	For any $s<t$, $y\in K_R$, let $r<dist(y,\partial K_R)$ \textcolor{red}{and $r\le C\sqrt{t}$}. The parabolic Green's function satisfies \textcolor{red}{[specify $C$ and $\alpha$]}
	\begin{equation*}
		\norm{\nabla_{\bz} \Gamma(\bx,t;\cdot,\cdot)}_{L^2\left(Q_r(\by,s)\right)}^2
%		\le
%		\int_{s-r^2}^{s}
%		\int_{B_{r}(y)\cap K_R} \abs{\nabla_{\bz} \Gamma(\bx,t;\bz,\tau)}^2 \,d\bz 
%		\,d\tau
		\le
		C r^{d} \frac{1}{(t-s)^d}\exp\left(-\alpha \frac{\abs{x-y}^2}{t-s}\right).
	\end{equation*}
\end{lemma}
\begin{proof}
	We now notice that, since the coefficients are homogeneous in time, the Green's function does only depend on the \emph{difference} between $t$ and $s$, so we can write
	\begin{equation*}
		G(x,t-s;y) := \Gamma(x,t;y,s)
	\end{equation*}
	to simplify the notation. 
	Moreover, from the symmetry in the $x$ and $y$ arguments, $G(x,t;y)=G(y,t;x)$\footnote{The symmetry in $x$ and $y$ could be proven as follows:
		\begin{multline*}
				G(x,t;y)
				=\int_{\Omega} G(z,t;y)G(z,0;x)\,dz
				=\frac{1}{2}\int_0^{\infty}\int_{\Omega} G(z,t;y)G(z,t;x)\,dz\\
				=\int_{\Omega} G(z,0;y)G(z,t;x)\,dz
				=G(y,t;x).
		\end{multline*}}, we deduce that
	\begin{equation*}
		\nabla_y G(x,t;y)= \nabla_y G(y,t;x).
	\end{equation*}
	By applying the parabolic Caccioppoli's inequality on $\nabla_y G(\cdot,\cdot;x)$
	\begin{equation*}
		\begin{aligned}
			\int_{s-r^2}^{s}
			\int_{B_{r}(y)} \abs{\nabla_{\bz} \Gamma(\bx,t;\bz,\tau)}^2 \,d\bz 
			\,d\tau
			&=
			\int_{t-s}^{t-s+r^2}
			\int_{B_{r}(y)} \abs{\nabla_{\bz} G(\bz,\tau;\bx)}^2 \,d\bz \,d\tau \\
			&\le\frac{C}{r^2}
			\int_{t-s}^{t-s+4r^2}
			\int_{B_{2r}(y)} \abs{G(\bz,\tau;\bx)}^2 \,d\bz \,d\tau.
		\end{aligned}
	\end{equation*}
	Finally, by recalling the Nash-Aronson estimate:
	\begin{equation*}
		\begin{aligned}
			\int_{s-r^2}^{s}
			\int_{B_{r}(y)} \abs{\nabla_{\bz} \Gamma(\bx,t;\bz,\tau)}^2 \,d\bz 
			\,d\tau
			&\le
			\frac{C}{r^2}
			\int_{t-s}^{t-s+4r^2}
			\int_{B_{2r}(y)} \abs{G(\bz,\tau;\bx)}^2 \,d\bz \,d\tau\\
			\text{\footnotemark} &\le
			C r^{d} \frac{1}{(t-s)^d}\exp\left(-\alpha \frac{\abs{x-y}^2}{t-s}\right).
		\end{aligned}
	\end{equation*}
\footnotetext{See also Proposition 3.3, Ref. \refcite{DKN09} and Proposition E.1 Ref. \refcite{AKM19} for a proof of the same result for the fundamental solution of the parabolic equation.}
\end{proof}

We are now ready to prove \cref{lemma: preliminary estimate sup-theta}.
\begin{proof}[\cref{lemma: preliminary estimate sup-theta}]
By applying the H\"older inequality to the identity \cref{eq:theta through green flux2} and from the boundedness of $a(\by)$ we have that
\begin{multline}\label{eq:initial estimate theta}
	\abs{\theta^i(\bx,t)} = \abs{ \int_{0}^{t} \int_{\partial K_R} \mathbf{n} \cdot a(\by) \nabla_{\by} \Gamma(\bx,t;\by,s) v^i(\by,s)  \,d\sigma_\by\,ds }\\
	\le \beta \norm{v^i}_{L^2\left((0,t)\times\partial K_R\right)}
	\left(
	\int_{0}^{t} 
	\int_{\partial K_R} \abs{\nabla_{\by} \Gamma(\bx,t;\by,s)}^2  \,d\sigma_\by\,ds
	\right)^{1/2}.
\end{multline}
We start by bounding the term $\norm{v^i}_{L^2\left((0,t)\times\partial K_R\right)}$.
The value of $\norm{ v^i(\cdot,s) }_{L^2(\partial K_R)} $ is well defined for any time $s>0$ and we can estimate it by the following inequality 
\begin{equation*}
	\norm{ v^i(\cdot,s) }_{L^2(\partial K_R)} = \norm{ v^i(\cdot,s)(1 - \rho) }_{L^2(\partial K_R)} \le C_{tr} 
	%\norm{\nabla \left( v^i(\cdot,s)(1 - \rho) \right) }_{L^2(\Delta)}.
	\norm{ v^i(\cdot,s)(1 - \rho)  }_{H^1(\Delta)},
\end{equation*}
where $C_{tr}$ is fixed, thanks to the fact that the distance between $K_{\tilde{R}}$ and $\partial K_R$ is larger or equal to $1/2$.
As $\rho\in C^1(K_R)$ and $\partial_{x_k} v^i(\cdot,s) \in L^2(K_R)$ the product rule holds and we can write
\begin{equation*}
	\norm{\nabla( v^i(1-\rho))}_{L^2(\Delta)} \le \norm{\nabla v^i}_{L^2(\Delta)} + \norm{\nabla \rho}_{L^{\infty}(\Delta)} \norm{v^i}_{L^2(\Delta)}.
\end{equation*}
Let us now consider a covering of $\Delta$, defined as $\Delta_K:=  \bigcup_{\by\in\partial K_{\frac{R + \tilde{R}}{2}}} K+\by$. Then, $\abs{\Delta_K}= c(d) \abs{\partial K_{\frac{R + \tilde{R}}{2}}} \mathrm{diam}(K) \le C R^{d-1}$.
By exploiting the periodic structure of $v^i$ we have that 
\begin{multline*}%\label{eq: estimate v boundary}
	\norm{v^i}_{L^2(\Delta)}
	\le 
	\norm{v^i}_{L^2(\Delta_K)}
	\le
	\left(\frac{\abs{\Delta_K}}{\abs{K}}\right)^{1/2}\norm{v^i}_{L^2(K)}, \\
	%\quad 
	\norm{\nabla v^i}_{L^2(\Delta)}
	\le 
	\norm{\nabla v^i}_{L^2(\Delta_K)}
	\le 
	\left(\frac{\abs{\Delta_K}}{\abs{K}}\right)^{1/2}\norm{\nabla v^i}_{L^2(K)}.
\end{multline*}
Finally, we recall that in the space $W^1_{per}(K)$ the Poincar\'e-Wirtinger inequality holds:
\begin{equation*}
	\norm{v^i}_{L^2(K)} \le C_P \Lnorm{\nabla v^i}{K}
\end{equation*}
so that 
\begin{equation*}
	\begin{split}
		\Lnorm{v^i(\cdot,s)}{\partial K_R}
		&\le 
		C_{tr} C_{\rho} C_P \left(\frac{\abs{\Delta}}{\abs{K}}\right)^{1/2}\norm{\nabla v^i(\cdot,s)}_{L^2(K)} \\
		&\le C
		R^{\frac{d-1}{2}} \norm{\nabla v^i(\cdot,s)}_{L^2(K)}.
	\end{split}	
\end{equation*}
In conclusion, by standard energy estimates on the solution of parabolic equations, the $L^2\left((0,t)\times\partial K_R\right)$-norm of $v^i$ is bounded by
\begin{equation}\label{eq: estimate f 1 copy}
\begin{aligned}
\Lnorm{v^i}{(0,t)\times\partial K_R}
&\le C
R^{\frac{d-1}{2}} \Lnorm{\nabla v^i}{(0,t)\times K}\\
&\le \frac{C}{\sqrt{2\alpha}}
R^{\frac{d-1}{2}} \Lnorm{\nabla\cdot\left(a\mathbf{e}_i\right)}{K}.
\end{aligned}
\end{equation}


%Now, we move to the estimation of the $L^2$-$L^2$ norm of the gradient of the parabolic Green's function. Our strategy relies on the use of the parabolic Caccioppoli inequality, stated in the following \Cref{lemma: caccioppoli} and proved, e.g., in \S 1, Chapter 8, Ref. \refcite{AKM19}.
%\begin{lemma}\label{lemma: caccioppoli}
%	Let $u\in L^2\left((t-4r^2,t),H^1\left(B_{2r}(\bx)\right)\right)$ solve
%	\begin{equation*}
%		\partial_t u - \nabla\cdot\left(a(\bx)\nabla u \right)=0, \quad \text{in }(t-4r^2,t)\times B_2r(\bx).
%	\end{equation*}
%	There exists a constant $C(d,\alpha,\beta)\le \infty$ such that
%	\begin{equation*}%\label{eq:caccioppoli inequality}
%		\norm{\nabla u}_{L^2\left((t-r^2,t)\times B_{r}(x)\right)}
%		\le
%		C \norm{u}_{L^2\left((t-4r^2,t)\times B_{2r}(x)\right)}.
%	\end{equation*}
%\end{lemma}

We now aim to use the bound on $\norm{\nabla_{\by}\Gamma(\bx,t;\cdot,\cdot)}_{Q_r(\by,s)}$, developed in \cref{lemma:bound gradient green}, to control the last term in \eqref{eq:initial estimate theta}. In order to do so, we first have to rewrite the double integral in \cref{eq:initial estimate theta} by a covering argument:
\begin{multline}
	\label{eq:covering argument}
	\int_{0}^{t}  
	\int_{\partial K_R} \abs{\nabla_{\by} \Gamma(\bx,t;\by,s)}^2  \,d\sigma_\by \,ds\\
	\le C 
	\int_{0}^{t}  
	\int_{\partial K_R}
	\frac{1}{r^2}
	\int_{s-r^2}^{s}  
	 \frac{1}{\abs{B_{r}(y)\cap K_R}}
	\int_{B_{r}(y)\cap K_R} \abs{\nabla_{\bz} \Gamma(\bx,t;\bz,\tau)}^2 \,d\bz   \,d\tau \,d\sigma_\by \,ds\\
	\le C
	\int_{0}^{t}  
	\int_{\partial K_R}
	r^{-d-2}  
	\int_{s-r^2}^{s}
	\int_{B_{r}(y)\cap K_R} \abs{\nabla_{\bz} \Gamma(\bx,t;\bz,\tau)}^2 \,d\bz \,d\tau \,d\sigma_\by  \,ds
\end{multline}
where $C=C(d)$ and we assumed that $2r\le R-\tilde{R}$, so that $B_{r}(y)\cap K_R\subset \Delta$ (being $y\in \partial K_R$).\textcolor{red}{ We kept the term $r^{-d-2}$ \emph{inside} the integral is $s$ because we might have to choose $r=r(s)$.}

\begin{remark}
	The above integral ``expansion'' does make sense only if $\abs{\nabla\Gamma}$ is continuous in a neighbourhood of the boundary.
\end{remark}
%We now notice that, since the coefficients are homogeneous in time, the Green's function does only depend on the \emph{difference} between $t$ and $s$, so we can write
%\begin{equation*}
%	G(x,t-s;y) := \Gamma(x,t;y,s)
%\end{equation*}
%to simplify the notation. 
%Moreover, from the symmetry in the $x$ and $y$ arguments, $G(x,t;y)=G(y,t;x)$\footnote{\textcolor{red}{I did not find any reference about the symmetry of the Green's function for parabolic boundary value problems. However, we know that the Green's function for elliptic BVPs is symmetric in its arguments and that the time integral of the parabolic Green's function is the elliptic one. If the parabolic Green's function was not symmetric, the elliptic one would not be either, thus having a contradiction.}}, we deduce that
%\begin{equation*}
%	\nabla_y G(x,t;y)= \nabla_y G(y,t;x).
%\end{equation*}
%In the following part we derive explicit bound for the inner double integral by using \Cref{lemma: caccioppoli}, whose proof can be found in \S 1, Chapter 8, Ref. \refcite{AKM19}.
%\begin{multline*}
%	\int_{s-r^2}^{s}
%	\int_{B_{r}(y)\cap K_R} \abs{\nabla_{\bz} \Gamma(\bx,t;\bz,\tau)}^2 \,d\bz 
%	\,d\tau\\
%	=
%	\int_{s-r^2}^{s}
%	\int_{B_{r}(y)\cap K_R} \abs{\nabla_{\bz} G(\bx,t-\tau;\bz)}^2 \,d\bz \,d\tau \\
%	=
%	\int_{t-s}^{t-s+r^2}
%	\int_{B_{r}(y)\cap K_R} \abs{\nabla_{\bz} G(\bz,\tau;\bx)}^2 \,d\bz \,d\tau \\
%	\le
%	\int_{t-s}^{t-s+4r^2}
%	\int_{B_{2r}(y)\cap K_R} \abs{G(\bz,\tau;\bx)}^2 \,d\bz \,d\tau.
%\end{multline*}
%
%%
%%Thus the first step is to estimate $\int_{B_{r}(y)\cap K_R} \abs{\nabla_{\bz} \Gamma(\bx,t;\bz,s)}^2 \,d\bz$. The idea is to use the following lemma which can be found in Ref. \refcite{AKM19}, Chapter 8.
%%\begin{lemma} \label{lemma: time slice gradient}
%%	Let $u\in L^2\left((t-4r^2,t),H^1\left(B_{2r}(\bx)\right)\right)$ solve
%%	\begin{equation*}
%%		\partial_t u - \nabla\cdot\left(a(\bx)\nabla u \right)=0, \quad \text{in }(t-4r^2,t)\times B_2r(\bx).
%%	\end{equation*}
%%There exists a constant $C(d,\alpha,\beta)\le \infty$ such that 
%%\begin{equation}\label{eq:time slice estimate}
%%	\sup_{s \in (t-r^2,t)} \norm{\nabla u(\cdot,s)}_{L^2\left(B_{r}(x)\right)}
%%	\le
%%	\frac{C}{2r} \norm{\nabla u(\cdot,s)}_{L^2\left((t-4r^2,t)\times B_{2r}(x)\right)}.
%%\end{equation}
%%\end{lemma}
%%\begin{lemma}\label{lemma: caccioppoli}
%%	Let $u\in L^2\left((t-4r^2,t),H^1\left(B_{2r}(\bx)\right)\right)$ solve
%%	\begin{equation*}
%%		\partial_t u - \nabla\cdot\left(a(\bx)\nabla u \right)=0, \quad \text{in }(t-4r^2,t)\times B_2r(\bx).
%%	\end{equation*}
%%	There exists a constant $C(d,\alpha,\beta)\le \infty$ such that
%%	\begin{equation}\label{eq:caccioppoli inequality}
%%		\norm{\nabla u}_{L^2\left((t-r^2,t)\times B_{r}(x)\right)}
%%		\le
%%		C \norm{u}_{L^2\left((t-4r^2,t)\times B_{2r}(x)\right)}.
%%	\end{equation}
%%\end{lemma}
%Finally, by recalling the Nash-Aronson estimate on the Green function\footnote{The Nash-Aronson estimate is usually given for the infinite domain Green's function, but it is also valid for the bounded domain one with Dirichlet boundary conditions, thanks to the maximum principle.}:
%\begin{multline*}
%	\int_{s-r^2}^{s}
%	\int_{B_{r}(y)\cap K_R} \abs{\nabla_{\bz} \Gamma(\bx,t;\bz,\tau)}^2 \,d\bz 
%	\,d\tau\\
%	\le
%	\int_{t-s}^{t-s+4r^2}
%	\int_{B_{2r}(y)\cap K_R} \abs{G(\bz,\tau;\bx)}^2 \,d\bz \,d\tau\\
%	{\color{red}{\text{MAKE SURE THIS IS CLEAR}}}\le
%	C r^{d+2} \frac{1}{(t-s)^d}\exp\left(-\alpha \frac{\abs{x-y}^2}{t-s}\right).
%\end{multline*}
Then, by recalling the result of \cref{lemma:bound gradient green}:
\begin{multline}
	\int_{0}^{t}  
	\int_{\partial K_R} \abs{\nabla_{\by} \Gamma(\bx,t;\by,s)}^2  \,d\sigma_\by \,ds
	\le C
	\int_{0}^{t}  
	\int_{\partial K_R} 
	\frac{1}{r^2} \frac{1}{(t-s)^d}\exp\left(-\alpha \frac{\abs{x-y}^2}{t-s}\right)
	 \,d\sigma_\by  \,ds\\
	 \le 
	 C \abs{\partial K_R} 
	 \int_{0}^{t} 
	 \frac{1}{r^2} \frac{1}{(t-s)^d}\exp\left(-\alpha \frac{\abs{x-y}^2}{t-s}\right)\,ds\\
	 \le
	 C \frac{1}{r^2} R^{d-1} \abs{R-L}^{2-2d} \left(\frac{\abs{R-L}^2}{t}\right)^{d-2} \exp\left(-\alpha\frac{\abs{R-L}^2}{t}\right).
\end{multline}
By the result above and \eqref{eq: integral abs theta 1 copy}, we conclude that 
\begin{multline}
	\abs{\theta^i(\bx,t)} 
	\le
	C \frac{1}{r^2}
	R^{\frac{d-1}{2}} \norm{\nabla v^i(\cdot,s)}_{L^2\left((0,t),L^2(K)\right)}
	\frac{R^{\frac{d-1}{2}}}{\abs{R-L}}
	\frac{1}{t^{d/2-1}} \exp\left(-\alpha\frac{\abs{R-L}^2}{t}\right)\\
	\le C \frac{1}{r^2}
	\frac{R^{d-1}}{\abs{R-L}}  \frac{1}{t^{d/2-1}} \exp\left(-\alpha\frac{\abs{R-L}^2}{t}\right),
\end{multline}
where $C$ depends on $\alpha,\beta,d$.
\textcolor{red}{[Does $r$ depend on $s,t$? How?]}
\end{proof}
